Efficient Conformal Prediction via Cascaded Inference with Expanded Admission

In this paper, we present a novel approach for conformal prediction (CP), in which we aim to identify a set of promising prediction candidates -- in place of a single prediction. This set is guaranteed to contain a correct answer with high probability, and is well-suited for many open-ended classification tasks. In the standard CP paradigm, the predicted set can often be unusably large and also costly to obtain. This is particularly pervasive in settings where the correct answer is not unique, and the number of total possible answers is high. We first expand the CP correctness criterion to allow for additional, inferred "admissible" answers, which can substantially reduce the size of the predicted set while still providing valid performance guarantees. Second, we amortize costs by conformalizing prediction cascades, in which we aggressively prune implausible labels early on by using progressively stronger classifiers -- again, while still providing valid performance guarantees. We demonstrate the empirical effectiveness of our approach for multiple applications in natural language processing and computational chemistry for drug discovery.

==> sections/broader_impact.tex <==
\section*{Broader Impact}

This work aims to improve two important aspects of conformal prediction for classification, namely, \emph{predictive} and \emph{computational} efficiency. In doing so, this work brings us closer to achieving practically usable classifiers with strong performance guarantees---a quality that is critical to many important applications. For example, in this work we applied our methods to information retrieval for fact verification, question answering, and computational chemistry for drug discovery (in-silico screening tools). We acknowledge that companies for which these types of tasks are particularly important---e.g., pharmaceutical companies in terms of the drug discovery setting---could stand to asymmetrically gain from a successful implementation of our work, but not unfairly so. The primary factors contributing to a failed system are the same for all standard conformal predictions, namely: (1) violations of the exchangeability assumption (resulting in invalid CPs), or (2) low statistical power in the nonformity measure (resulting in low predictive efficiency). The consequence of a failed system is primarily decreased utility as a precise prediction service, and ultimately, its use would simply be discontinued.

==> sections/scratch.tex <==
  Providing the correct answer among a small set of suggestions is... (motivation for cp).
    Conformal Prediction (CP) guarantees a set of predictions that with high probability contains a correct answer. However, this might come at the cost of low efficiency, i.e., a large set of positive predictions. In this work, we develop methods to improve the efficiency of the predicted set while preserving the validity guarantee. We construct a cascaded pipeline that relies on the characteristics of CP in order to early-reject implausible predictions by a simple classifier and to leverage the efficacy of a stronger classifier. We show that this approach can both (1) increase the performance by combining complementary signals and (2) reduce the computational effort of applying a complex classifier on a large label set. In addition, we 
    
    
Given a tolerance level $\epsilon$, Conformal Prediction is framework for producing a set of suggestions that contains the true answer with probability $1 - \epsilon$---in finite samples, and without making distributional assumptions.

Providing a small set of suggestions in place of a single prediction is well-suited for many open-ended applications. Given a tolerance level $\epsilon$, Conformal Prediction (CP) is a technique for producing a ``valid'' set of predictions that contains the true answer with probability $1 - \epsilon$---in finite samples, and without making distributional assumptions. In practice, however, during inference standard CP can suffer from both low \emph{predictive} and \emph{computational} efficiency---i.e., the predicted set is both loose and costly to obtain. This is particularly pervasive in settings where the correct answer is not unique, and the number of total possible answers is large. In this work, we develop two complementary and simple yet effective techniques for improving both types of efficiencies. First, we generalize CP validity to allow for arbitrary measures of success---allowing our framework to make more aggressive predictions while remaining ``equivalently correct'' (EC) in open-ended problems. Second, we conformalize prediction cascades to amortize computational cost by pruning implausible labels using progressively stronger classifiers, while still guaranteeing valid equivalent correctness. We demonstrate the effectiveness of our approach for multiple end tasks.
